Lambda theories of effective lambda models

A longstanding open problem is whether there exists a non-syntactical model of untyped lambda-calculus whose theory is exactly the least equational lambda-theory (=Lb). In this paper we make use of the Visser topology for investigating the more general question of whether the equational (resp. order) theory of a non syntactical model M, say Eq(M) (resp. Ord(M)) can be recursively enumerable (= r.e. below). We conjecture that no such model exists and prove the conjecture for several large classes of models. In particular we introduce a notion of effective lambda-model and show that for all effective models M, Eq(M) is different from Lb, and Ord(M) is not r.e. If moreover M belongs to the stable or strongly stable semantics, then Eq(M) is not r.e. Concerning Scott's continuous semantics we explore the class of (all) graph models, show that it satisfies Lowenheim Skolem theorem, that there exists a minimum order/equational graph theory, and that both are the order/equ theories of an effective graph model. We deduce that no graph model can have an r.e. order theory, and also show that for some large subclasses, the same is true for Eq(M).

==> macro-duecolonne.tex <==
% Macro di Giulio

\newcommand{\cardinality}[1]{card(#1)}% cardinality of a set 
\newcommand{\codepair}[2]{<#1,#2>}% code of a pair
\newcommand{\codepairmix}[2]{\ll #1,#2 \gg}% code of a pair N^* X N
\newcommand{\Visser}[1]{\mathscr{V}_{#1}}
\newcommand{\restr}{\upharpoonright}% restriction
\newcommand{\Kdn}[1]{\widehat{#1}}% restriction
\newcommand{\emptyrho}{\rho_\bot}% empty environment
\newcommand{\RE}{{\mathcal R}{\mathcal E}}% r.e. sets
\newcommand{\CORE}{{\mathcal R}{\mathcal E}^{co}}% co-r.e.
\newcommand{\Kleeneq}{\simeq}% Kleene equivalence
\newcommand{\Zero}{\textrm{Zero}}
\newcommand{\Pred}{\textrm{Pred}}
\newcommand{\Succ}{\textrm{Succ}}
\newcommand{\ecomp}{\zeta}
\newcommand{\st}{:}
\newcommand{\pow}[1]{\mathscr{P}(#1)}
\newcommand{\Intunder}[1]{\Lambda^o_{#1}}
\newcommand{\Prime}[1]{\cP(#1)}
\newcommand{\step}[2]{\varepsilon_{#1,#2}}
\newcommand{\D}{{\mathcal D}}
\newcommand{\E}{{\mathcal E}}
\newcommand{\std}[1]{\underline{#1}}
\newcommand{\cod}[1]{\ulcorner #1 \urcorner}
\newcommand{\vphi}{\varphi}
%\newcommand{\partarrow}{\rightharpoonup_p}
\newcommand{\partarrow}{\rightharpoonup}
\newcommand{\W}{{\cal W}}
\newcommand{\App}{\cA}
\newcommand{\Abs}{\lambda}
\newcommand{\compl}[1]{#1^c}
\newcommand{\domcomp}[1]{#1^{comp}}
\newcommand{\domdec}[1]{#1^{dec}}
\newcommand{\Intcomp}[1]{\vert #1\vert^{comp}}
\newcommand{\Int}[1]{\vert #1\vert}
\newcommand{\clup}[1]{#1\hspace{-5pt}\uparrow}
\newcommand{\cldn}[1]{#1\hspace{-5pt}\downarrow}
\newcommand{\inv}[1]{#1^{-}}
\newcommand{\img}[1]{#1^{+}}
%\renewcommand{\sup}[1]{\bigvee #1}
\renewcommand{\sup}[1]{\bigsqcup #1}
\newcommand{\Unsolvable}{\mathscr{U}}
\newcommand{\cl}[1]{\overline{#1}}
\newcommand{\seq}[1]{\overline{#1}}
\newcommand{\const}[1]{\underline{#1}}
\newcommand{\intrho}[1]{|#1|^i_\rho}
\renewcommand{\bold}[1]{{\bf #1}}
\newcommand{\compel}[1]{{\bf {\cal K}}(#1)}
\newcommand{\Appr}[1]{\c App(\textrm{$#1$})}
\newcommand{\imp}{\Rightarrow}
\newcommand{\sqle}{\sqsubseteq}
\newcommand{\BTle}{\sqsubseteq}
\newcommand{\BTeq}{=}
\newcommand{\BTsup}{\bigsqcup}
%\newcommand{\nat}{\mathbb{\omega}}
\newcommand{\nat}{\mathbb{N}}
\newcommand{\BT}{\mathcal{BT}}
\newcommand{\Base}{\mathcal{O}}

% Macro di Nino

\newtheorem{theorem}{Theorem}[section]
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{subclaim}[theorem]{Subclaim}
\newtheorem{example}[theorem]{Example}

%
\newcommand{\ot}{\overline{t}}
\newcommand{\os}{\overline{s}}
\newcommand{\sskV}{{\bf k}\sp {\bf V}}
\newcommand{\sssV}{{\bf s}\sp{\bf V}}
\newcommand{\glV}{{\gl^{\bf V}}}
\newcommand{\cdotV}{\cdot^{\bf V}}
\newcommand{\cterm}{combinatory term}
\newcommand{\bZd}{\mbox{\bf Zd\,}}
\newcommand{\Cr}{\mbox{\rm Cr\,}}
\newcommand{\ConA}{{\bf C}{\rm on}\hspace{.01in}{\bf A}}
\newcommand{\ConB}{{\bf C}{\rm on}\hspace{.01in}{\bf B}}
\newcommand{\ConAB}{{\bf C}{\rm on}\hspace{.01in}({\bf A}$\times${\bf B})}
\newcommand{\lvar}{$\gl$-variable}
\newcommand{\bI}{{\bf I }}
%\newcommand{\qed}{$\Box$}
\newcommand{\TolA}{{\bf T}{\rm ol}\hspace{.01in}{\bf A}}
\newcommand{\FRA}{FR\hspace{.01in}{\bf A}}
\newcommand{\bnew}{\marginpar{\mbox{$\top$}}}
\newcommand{\enew}{\marginpar{\mbox{$\bot$}}}
\newcommand{\snew}{\marginpar{\mbox{$\leftarrow$}}}
\newcommand{\fnew}{\marginpar{\mbox{$\downarrow$}}}
\newcommand{\glxA}{\gl x^{\bA}}
\newcommand{\Zd}{\mbox{\rm Zd\,}}
% theorem-like commands
%

%\newtheorem{claim}{Claim}[section]
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{corollary}{Corollary}[section]
%\newtheorem{definition}{Definition}
%\newtheorem{definition}{Definition}[section]
%\newtheorem{proposition}{Proposition}[section]
%\newtheorem{lemma}{Lemma}[section]
%\newtheorem{example}{Example}[section]

\newtheorem{claimsub}{Claim}[subsection]
\newtheorem{theoremsub}{Theorem}[subsection]
\newtheorem{corollarysub}{Corollary}[subsection]
%\newtheorem{definition}{Definition}
\newtheorem{definitionsub}{Definition}[subsection]
\newtheorem{propositionsub}{Proposition}[subsection]
\newtheorem{lemmasub}{Lemma}[subsection]
\newtheorem{examplesub}{Example}[subsection]

\newtheorem{claimsubsub}{Claim}[subsubsection]
\newtheorem{theoremsubsub}{Theorem}[subsubsection]
\newtheorem{corollarysubsub}{Corollary}[subsubsection]
%\newtheorem{definition}{Definition}
\newtheorem{definitionsubsub}{Definition}[subsubsection]
\newtheorem{propositionsubsub}{Proposition}[subsubsection]
\newtheorem{lemmasubsub}{Lemma}[subsubsection]
\newtheorem{examplesubsub}{Example}[subsubsection]

\newcommand{\Over}[1]{\raisebox{-1.6mm}{{\scriptsize #1}}}
\newcommand{\SubOver}[1]{\raisebox{-0.6mm}{{\tiny #1}}}

\newcommand{\FOL}{\mbox{$L_{\omega,\omega}$}}

%\newcommand{\And}{\mbox{$\wedge$}}
\newcommand{\Or}{\mbox{$\vee$}}
\newcommand{\Neg}{\mbox{$\neg$}}
\newcommand{\noteq}{\mbox{$\neq$}}
\newcommand{\fiproof}{\mbox{$(\Rightarrow)$}}
\newcommand{\ifproof}{\mbox{$(\Leftarrow)$}}
\newcommand{\of}{\mbox{$\in$}}
\newcommand{\notof}{\mbox{$\not\in$}}
\newcommand{\union}{\mbox{$\cup$}}
\newcommand{\intersection}{\mbox{$\cap$}}
\newcommand{\except}{\mbox{$-$}}
\newcommand{\cardof}[1]{\mbox{$|$}#1\mbox{$|$}}
\newcommand{\forevery}{\mbox{$\forall$}}
\newcommand{\therexists}{\mbox{$\exists$}}
\newcommand{\within}{\mbox{$\subseteq$}}
\newcommand{\includes}{\mbox{$\supseteq$}}
\newcommand{\product}{\mbox{$\times$}}
\newcommand{\Power}{\mbox{$\wp$}}
\newcommand{\Powernonempty}{\Power\mbox{$_{+}$}}
\newcommand{\yields}{\mbox{$\mapsto$}}
\newcommand{\comp}{\mbox{$\circ$}}
\newcommand{\emptys}{\mbox{$\emptyset$}}
\newcommand{\emptypres}{\emptys}
\newcommand{\nonabove}{\mbox{$\preceq$}}
\newcommand{\fullynonabove}{\mbox{$\sqsubseteq$}}
\newcommand{\classicallynonabove}{\mbox{$\leq$}}
\newcommand{\carrierof}[1]{\mbox{$|$}#1\mbox{$|$}}
\newcommand{\setof}[1]{\mbox{$\{$}#1\mbox{$\}$}}
\newcommand{\suchthat}{\mbox{$|$}}
\newcommand{\unionall}[3]{\mbox{$\bigcup_{#1\in#2}$}#3}
\newcommand{\widunionall}[3]{\parbox[t]{#3}
                         {\centering\mbox{$\bigcup$}
                          \\ \protect\vspace*{-1.5mm}
                          {\scriptsize #1\of#2}}}
\newcommand{\intsnall}[3]{\mbox{$\bigcap_{#1\in#2}$}#3}
\newcommand{\widintsnall}[3]{\parbox[t]{#3}
                         {\centering\mbox{$\bigcap$}
                          \\ \protect\vspace*{-1.5mm}
                          {\scriptsize #1\of#2}}}
\newcommand{\ifamily}[3]{\setof{#1\mbox{$_{#2}$}}\mbox{$_{#2\in#3}$}}
\newcommand{\indx}{{\it j}}
\newcommand{\anindx}{{\it k}}
\newcommand{\indxset}{{\it J}}
\newcommand{\iso}{\mbox{$\simeq$}}
\newcommand{\lweq}{\mbox{$\leq$}}
\newcommand{\greq}{\mbox{$\geq$}}
\newcommand{\grth}{\mbox{$>$}}
\newcommand{\eqdef}{\mbox{$\stackrel{\it def}{=}$}}
\newcommand{\inverseof}[1]{#1\mbox{$^{-1}$}}
\newcommand{\minverseof}[1]{#1^{-1}}

\newcommand{\seqof}[3]{#1\mbox{$_{1}$}#2\ldots#2#1\mbox{$_{#3}$}}

\newcommand{\seqSubOverof}[3]{#1\raisebox{-2.2mm}
                                     {{\tiny 1}}#2\ldots#2#1\raisebox{-2.2mm}
                                                                 {{\tiny #3}}}

\newcommand{\rpsreq}{(\dag)}
\newcommand{\epsreq}{(\ddag)}
\newcommand{\satinv}{(\S)}
\newcommand{\adequacy}{(\S\S)}
\newcommand{\fulladequacy}{(\S\S\S)}
\newcommand{\finitarity}{(\pounds)}

\newcommand{\upar}{\uparrow}
\newcommand{\Upar}{\Uparrow}
\newcommand{\doar}{\downarrow}
\newcommand{\Doar}{\Downarrow}

\newcommand{\riar}{\rightarrow}
\newcommand{\lear}{\leftarrow}
\newcommand{\Riar}{\Rightarrow}
\newcommand{\Lear}{\Leftarrow}
\newcommand{\leriar}{\leftrightarrow}
\newcommand{\Leriar}{\Leftrightarrow}

\newcommand{\uC}{\underline {\bf C}}
\newcommand{\uD}{\underline {\bf D}}
\newcommand{\uE}{\underline E}
\newcommand{\ugS}{\underline\Sigma}
\newcommand{\uunion}{\underline\cup}
\newcommand{\ubigunion}{\underline\bigcup}
\newcommand{\unE}{\underline E}

\newcommand{\oE}{{\overline E}}
\newcommand{\oP}{{\overline P}}
\newcommand{\oV}{{\overline V}}
\newcommand{\oW}{{\overline W}}
\newcommand{\oU}{{\overline U}}
\newcommand{\oD}{{\overline D}}

\newcommand{\cA}{{\cal A}}
\newcommand{\cB}{{\cal B}}
\newcommand{\cC}{{\cal C}}
\newcommand{\cE}{{\cal E}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cG}{{\cal G}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cJ}{{\cal J}}
\newcommand{\cL}{{\cal L}}
\newcommand{\cM}{{\cal M}}
\newcommand{\cP}{{\cal P}}
\newcommand{\cR}{{\cal R}}
\newcommand{\cS}{{\cal S}}
\newcommand{\cT}{{\cal T}}
\newcommand{\cU}{{\cal U}}
\newcommand{\cV}{{\cal V}}

\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}

\newcommand{\sm}{\leadsto}
\newcommand{\sopra}[2]{\stackrel{#1}{#2}}

%definitions for \bf letters
\newcommand{\bb}{{\bf b}}
\newcommand{\bA}{{\bf A}}
\newcommand{\bB}{{\bf B}}
\newcommand{\bC}{{\bf C}}
\newcommand{\bD}{{\bf D}}
\newcommand{\bE}{{\bf E}}
\newcommand{\bF}{{\bf F}}
\newcommand{\bK}{{\bf K}}
\newcommand{\bM}{{\bf M}}
\newcommand{\bN}{{\bf N}}
\newcommand{\bP}{{\bf P}}
\newcommand{\bR}{{\bf R}}
\newcommand{\bS}{{\bf S}}
\newcommand{\bT}{{\bf T}}
\newcommand{\bU}{{\bf U}}
\newcommand{\bX}{{\bf X}}
\newcommand{\bRel}{{\bf Rel}}
\newcommand{\bx}{{\bf x }}

\newcommand{\bCX}{{{\bf C}[X]}}

%definitions for lower case greek letters
\newcommand{\ga}{\alpha}
\newcommand{\gb}{\beta}
\newcommand{\gam}{\gamma}
\newcommand{\gd}{\delta}
\newcommand{\gep}{\varepsilon}
\newcommand{\gz}{\zeta}
\newcommand{\geta}{\eta}
\newcommand{\gth}{\vartheta}
\newcommand{\gi}{\iota}
\newcommand{\gv}{\nu}
\newcommand{\gk}{\kappa}
\newcommand{\gl}{\lambda}
\newcommand{\gm}{\mu}
\newcommand{\gn}{\nu}
\newcommand{\gx}{\xi}
\newcommand{\gp}{\pi}
\newcommand{\gr}{\rho}
\newcommand{\gs}{\sigma}
\newcommand{\gt}{\tau}
\newcommand{\gu}{\upsilon}
\newcommand{\gph}{\varphi}
\newcommand{\gch}{\chi}
\newcommand{\gps}{\psi}
\newcommand{\go}{\omega}

\newcommand{\gG}{\Gamma}
\newcommand{\gF}{\Phi}
\newcommand{\gD}{\Delta}
\newcommand{\gT}{\Theta}
\newcommand{\gP}{\Pi}
\newcommand{\gX}{\Xi}
\newcommand{\gS}{\Sigma}
\newcommand{\gO}{\Omega}
\newcommand{\gL}{\Lambda}
\newcommand\LT{\mbox{\sf LT}}
\newcommand\sfB{\mbox{\sf B}}
\newcommand\DCAI{\mbox{\sf DCA}_I}
\newcommand\RFA{\mbox{\sf RFA}}
\newcommand\RFAI{\mbox{\sf RFA}_I}
\newcommand\RFAJ{\mbox{\sf RFA}_J}
\newcommand\LAA{\mbox{\sf LAA}}
\newcommand\LAAI{\mbox{\sf LAA}_I}
\newcommand\WLAI{\mbox{\sf LAA}_I^w}
\newcommand\SWLAI{\mbox{\sf LAA}_I^{sw}}
\newcommand\LIEI{\mbox{\sf LIE}_I}
\newcommand\CLAI{\mbox{\sf LAA}_I^c}
\newcommand\CLFAI{\mbox{\sf LFA}_I^c}
\newcommand\SLAI{\mbox{\sf LAA}_I^s}
\newcommand\SSLAI{\mbox{\sf LAA}_I^{cs}}
\newcommand\OLAAI{\mbox{\sf OLAA}_I}
\newcommand\LAAIE{\mbox{\sf LAA}_I^\eta}
\newcommand\LAAJ{\mbox{\sf LAA}_J}
\newcommand\BA{\mbox{\sf BA}}
\newcommand\GSA{\mbox{\sf GSA}}
\newcommand\RGA{\mbox{\sf RGA}}
\newcommand\GA{\mbox{\sf GA}}
\newcommand\K{\mbox{\sf K}}
\newcommand\G{\mbox{\sf G}}

\newcommand\FLA{\mbox{\sf FLA}}
\newcommand\FLAI{\mbox{\sf FLA}_I}
\newcommand\FLAJ{\mbox{\sf FLA}_J}
\newcommand\LFA{\mbox{\sf LFA}}
\newcommand\LFAI{\mbox{\sf LFA}_I}
\newcommand\LFAJ{\mbox{\sf LFA}_J}
\newcommand\CA{\mbox{\sf CA}}
\newcommand\LA{\mbox{\sf LA}}
\newcommand\LM{\mbox{\sf LM}}
\newcommand{\CL}{\mbox{ \sf CL}}

\newcommand\ssk{{\bf k}}
\newcommand\sss{{\bf s}}
\newcommand\ssm{\mbox{\boldmath $m$}}
\newcommand\ssi{{\bf i}}
\newcommand\ssl{\mbox{\boldmath $l$}}
\newcommand\sso{\mbox{\boldmath $1$}}
\newcommand\sst{\mbox{\boldmath $2$}}
\newcommand\ssT{\mbox{\boldmath $T$}}
\newcommand\ssF{\mbox{\boldmath $F$}}
\newcommand\ccc{\mbox{\boldmath $c$}}

\newcommand\Con{\mbox{Con}}

\newcommand\sbA{{\mbox{\bf A}}}%
\newcommand\ssbA{{\mbox{\footnotesize\bf A}}}%
\newcommand\sbB{\mbox{\boldmath $B$}}%
\newcommand\sbC{{\mathbf C}}%
\newcommand\sbD{\mbox{\boldmath $D$}}%
\newcommand\sbE{\mbox{\boldmath $E$}}%
\newcommand\sbF{{\mbox{\bf F}}}%
\newcommand\sbG{\mbox{\boldmath $G$}}%
\newcommand\sbH{\mbox{\boldmath $H$}}%
\newcommand\sbI{\mbox{\boldmath $I$}}%
\newcommand\sbJ{\mbox{\boldmath $J$}}%
\newcommand\sbK{{\bold K}}%
\newcommand\sbL{{\bold L}}%
\newcommand\sbM{\mbox{\bf M}}%
\newcommand\sbN{\mbox{\bf N}}%
\newcommand\sbO{{\bold O}}%
\newcommand\sbP{{\bold P}}%
\newcommand\sbQ{{\bold Q}}%
\newcommand\sbR{{\bold R}}%
\newcommand\sbS{{\bold S}}%
\newcommand\sbT{{\bold T}}%
\newcommand\sbU{{\bold U}}%
\newcommand\sbV{{\bold V}}%
\newcommand\sbW{{\bold W}}%
\newcommand\sbX{{\bold X}}%
\newcommand\sbY{{\bold Y}}%
\newcommand\sbZ{{\bold Z}}%


\newcommand\oa{{\overline{a}}}
\newcommand\ob{{\overline{b}}}
\newcommand\oc{{\overline{c}}}
\newcommand\od{{\overline{d}}}
\newcommand\ox{{\overline{x}}}
\newcommand\oy{{\overline{y}}}
\newcommand\ou{{\overline{u}}}
\newcommand\ov{{\overline{v}}}
\newcommand\ow{{\overline{w}}}
\newcommand\oz{{\overline{z}}}
\newcommand\oQ{{\overline{Q}}}
\newcommand\oN{{\overline{N}}}
\newcommand\oM{{\overline{M}}}
\newcommand\oR{{\overline{R}}}
\newcommand\oX{{\overline{X}}}
\newcommand\ogx{{\overline{\gx}}}
\newcommand\oempty{{\overline{\emptyset}}}

\newcommand\twohead{{\twoheadrightarrow}}

\newcommand\up{{\uparrow}}
\newcommand\down{{\downarrow}}
\newcommand\updown{{\updownarrow}}

\newcommand{\bCI}{{\bC[I]}}
\newcommand{\bDI}{{\bD[I]}}

\newcommand\sseq{{\subseteq}}
\newcommand\arrow{{\to}}


==> macro-duecolonne11.tex <==
% Macro di Giulio

\newcommand{\Tins}[1]{#1^{\cT-ins}}
\newcommand{\cardinality}[1]{card(#1)}% cardinality of a set 
\newcommand{\codepair}[2]{\hspace{+2pt}<\hspace{-2pt}#1,#2\hspace{-3pt}>}% code of a pair
\newcommand{\codepairmix}[2]{\hspace{+2pt}\ll\hspace{-2pt} #1,#2 \hspace{-2.5pt}\gg}% code of a pair N^* X N
\newcommand{\Visser}[1]{\mathscr{V}_{#1}}
\newcommand{\restr}{\upharpoonright}% restriction
\newcommand{\Kdn}[1]{\widehat{#1}}% restriction
\newcommand{\emptyrho}{\rho_\bot}% empty environment
\newcommand{\RE}{{\mathcal R}{\mathcal E}}% r.e. sets
\newcommand{\CORE}{{\mathcal R}{\mathcal E}^{co}}% co-r.e.
\newcommand{\Kleeneq}{\simeq}% Kleene equivalence
\newcommand{\Zero}{\textrm{Zero}}
\newcommand{\Pred}{\textrm{Pred}}
\newcommand{\Succ}{\textrm{Succ}}
\newcommand{\ecomp}{\zeta}
\newcommand{\st}{:}
\newcommand{\pow}[1]{\mathscr{P}(#1)}
\newcommand{\Intunder}[1]{\Lambda^o_{#1}}
\newcommand{\Prime}[1]{\cP(#1)}
\newcommand{\step}[2]{\varepsilon_{#1,#2}}
\newcommand{\D}{{\mathcal D}}
\newcommand{\E}{{\mathcal E}}
\newcommand{\std}[1]{\underline{#1}}
\newcommand{\cod}[1]{\ulcorner #1 \urcorner}
\newcommand{\vphi}{\varphi}
%\newcommand{\partarrow}{\rightharpoonup_p}
\newcommand{\partarrow}{\rightharpoonup}
\newcommand{\W}{{\cal W}}
\newcommand{\App}{\cF}
\newcommand{\Abs}{\lambda}
\newcommand{\compl}[1]{#1^c}
\newcommand{\domcomp}[1]{#1^{comp}}
\newcommand{\domdec}[1]{#1^{dec}}
\newcommand{\Intcomp}[1]{\left|  #1\right|^{comp}}
\newcommand{\Int}[1]{\left|  #1\right|}
\newcommand{\clup}[1]{#1\hspace{-5pt}\uparrow}
\newcommand{\cldn}[1]{#1\hspace{-5pt}\downarrow}
\newcommand{\inv}[1]{#1^{-}}
\newcommand{\partinv}[1]{#1^{-1}}
\newcommand{\img}[1]{#1^{+}}
%\renewcommand{\sup}[1]{\bigvee #1}
\renewcommand{\sup}[1]{\bigsqcup #1}
\newcommand{\Unsolvable}{\mathscr{U}}
\newcommand{\cl}[1]{\overline{#1}}
\newcommand{\seq}[1]{\overline{#1}}
\newcommand{\const}[1]{\underline{#1}}
\newcommand{\intrho}[1]{|#1|^i_\rho}
\renewcommand{\bold}[1]{{\bf #1}}
\newcommand{\compel}[1]{{\bf {\cal K}}(#1)}
\newcommand{\Appr}[1]{\c App(\textrm{$#1$})}
\newcommand{\imp}{\Rightarrow}
\newcommand{\sqle}{\sqsubseteq}
\newcommand{\BTle}{\sqsubseteq_\cB}
\newcommand{\BTeq}{=}
\newcommand{\BTsup}{\bigsqcup}
%\newcommand{\nat}{\mathbb{\omega}}
\newcommand{\nat}{\mathbb{N}}
\newcommand{\BT}{\mathcal{BT}}
\newcommand{\Base}{\mathcal{O}}

% Macro di Nino
%\newtheorem{conjecture}{Conjecture}

%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{notation}[theorem]{Notation}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{claim}[theorem]{Claim}
%\newtheorem{subclaim}[theorem]{Subclaim}
%\newtheorem{example}[theorem]{Example}

%
\newcommand{\ot}{\overline{t}}
\newcommand{\os}{\overline{s}}
\newcommand{\sskV}{{\bf k}\sp {\bf V}}
\newcommand{\sssV}{{\bf s}\sp{\bf V}}
\newcommand{\glV}{{\gl^{\bf V}}}
\newcommand{\cdotV}{\cdot^{\bf V}}
\newcommand{\cterm}{combinatory term}
\newcommand{\bZd}{\mbox{\bf Zd\,}}
\newcommand{\Cr}{\mbox{\rm Cr\,}}
\newcommand{\ConA}{{\bf C}{\rm on}\hspace{.01in}{\bf A}}
\newcommand{\ConB}{{\bf C}{\rm on}\hspace{.01in}{\bf B}}
\newcommand{\ConAB}{{\bf C}{\rm on}\hspace{.01in}({\bf A}$\times${\bf B})}
\newcommand{\lvar}{$\gl$-variable}
\newcommand{\bI}{{\bf I }}
%\newcommand{\qed}{$\Box$}
\newcommand{\TolA}{{\bf T}{\rm ol}\hspace{.01in}{\bf A}}
\newcommand{\FRA}{FR\hspace{.01in}{\bf A}}
\newcommand{\bnew}{\marginpar{\mbox{$\top$}}}
\newcommand{\enew}{\marginpar{\mbox{$\bot$}}}
\newcommand{\snew}{\marginpar{\mbox{$\leftarrow$}}}
\newcommand{\fnew}{\marginpar{\mbox{$\downarrow$}}}
\newcommand{\glxA}{\gl x^{\bA}}
\newcommand{\Zd}{\mbox{\rm Zd\,}}
% theorem-like commands
%

%\newtheorem{claim}{Claim}[section]
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{corollary}{Corollary}[section]
%\newtheorem{definition}{Definition}
%\newtheorem{definition}{Definition}[section]
%\newtheorem{proposition}{Proposition}[section]
%\newtheorem{lemma}{Lemma}[section]
%\newtheorem{example}{Example}[section]

\newtheorem{claimsub}{Claim}[subsection]
\newtheorem{theoremsub}{Theorem}[subsection]
\newtheorem{corollarysub}{Corollary}[subsection]
%\newtheorem{definition}{Definition}
\newtheorem{definitionsub}{Definition}[subsection]
\newtheorem{propositionsub}{Proposition}[subsection]
\newtheorem{lemmasub}{Lemma}[subsection]
\newtheorem{examplesub}{Example}[subsection]

\newtheorem{claimsubsub}{Claim}[subsubsection]
\newtheorem{theoremsubsub}{Theorem}[subsubsection]
\newtheorem{corollarysubsub}{Corollary}[subsubsection]
%\newtheorem{definition}{Definition}
\newtheorem{definitionsubsub}{Definition}[subsubsection]
\newtheorem{propositionsubsub}{Proposition}[subsubsection]
\newtheorem{lemmasubsub}{Lemma}[subsubsection]
\newtheorem{examplesubsub}{Example}[subsubsection]

\newcommand{\Over}[1]{\raisebox{-1.6mm}{{\scriptsize #1}}}
\newcommand{\SubOver}[1]{\raisebox{-0.6mm}{{\tiny #1}}}

\newcommand{\FOL}{\mbox{$L_{\omega,\omega}$}}

%\newcommand{\And}{\mbox{$\wedge$}}
%\newcommand{\Or}{\mbox{$\vee$}}
\newcommand{\Neg}{\mbox{$\neg$}}
\newcommand{\noteq}{\mbox{$\neq$}}
\newcommand{\fiproof}{\mbox{$(\Rightarrow)$}}
\newcommand{\ifproof}{\mbox{$(\Leftarrow)$}}
\newcommand{\of}{\mbox{$\in$}}
\newcommand{\notof}{\mbox{$\not\in$}}
\newcommand{\union}{\mbox{$\cup$}}
\newcommand{\intersection}{\mbox{$\cap$}}
\newcommand{\except}{\mbox{$-$}}
\newcommand{\cardof}[1]{\mbox{$|$}#1\mbox{$|$}}
\newcommand{\forevery}{\mbox{$\forall$}}
\newcommand{\therexists}{\mbox{$\exists$}}
\newcommand{\within}{\mbox{$\subseteq$}}
\newcommand{\includes}{\mbox{$\supseteq$}}
\newcommand{\product}{\mbox{$\times$}}
\newcommand{\Power}{\mbox{$\wp$}}
\newcommand{\Powernonempty}{\Power\mbox{$_{+}$}}
\newcommand{\yields}{\mbox{$\mapsto$}}
\newcommand{\comp}{\mbox{$\circ$}}
\newcommand{\emptys}{\mbox{$\emptyset$}}
\newcommand{\emptypres}{\emptys}
\newcommand{\nonabove}{\mbox{$\preceq$}}
\newcommand{\fullynonabove}{\mbox{$\sqsubseteq$}}
\newcommand{\classicallynonabove}{\mbox{$\leq$}}
\newcommand{\carrierof}[1]{\mbox{$|$}#1\mbox{$|$}}
\newcommand{\setof}[1]{\mbox{$\{$}#1\mbox{$\}$}}
\newcommand{\suchthat}{\mbox{$|$}}
\newcommand{\unionall}[3]{\mbox{$\bigcup_{#1\in#2}$}#3}
\newcommand{\widunionall}[3]{\parbox[t]{#3}
                         {\centering\mbox{$\bigcup$}
                          \\ \protect\vspace*{-1.5mm}
                          {\scriptsize #1\of#2}}}
\newcommand{\intsnall}[3]{\mbox{$\bigcap_{#1\in#2}$}#3}
\newcommand{\widintsnall}[3]{\parbox[t]{#3}
                         {\centering\mbox{$\bigcap$}
                          \\ \protect\vspace*{-1.5mm}
                          {\scriptsize #1\of#2}}}
\newcommand{\ifamily}[3]{\setof{#1\mbox{$_{#2}$}}\mbox{$_{#2\in#3}$}}
\newcommand{\indx}{{\it j}}
\newcommand{\anindx}{{\it k}}
\newcommand{\indxset}{{\it J}}
\newcommand{\iso}{\mbox{$\simeq$}}
\newcommand{\lweq}{\mbox{$\leq$}}
\newcommand{\greq}{\mbox{$\geq$}}
\newcommand{\grth}{\mbox{$>$}}
\newcommand{\eqdef}{\mbox{$\stackrel{\it def}{=}$}}
\newcommand{\inverseof}[1]{#1\mbox{$^{-1}$}}
\newcommand{\minverseof}[1]{#1^{-1}}

\newcommand{\seqof}[3]{#1\mbox{$_{1}$}#2\ldots#2#1\mbox{$_{#3}$}}

\newcommand{\seqSubOverof}[3]{#1\raisebox{-2.2mm}
                                     {{\tiny 1}}#2\ldots#2#1\raisebox{-2.2mm}
                                                                 {{\tiny #3}}}

\newcommand{\rpsreq}{(\dag)}
\newcommand{\epsreq}{(\ddag)}
\newcommand{\satinv}{(\S)}
\newcommand{\adequacy}{(\S\S)}
\newcommand{\fulladequacy}{(\S\S\S)}
\newcommand{\finitarity}{(\pounds)}

\newcommand{\upar}{\uparrow}
\newcommand{\Upar}{\Uparrow}
\newcommand{\doar}{\downarrow}
\newcommand{\Doar}{\Downarrow}

\newcommand{\riar}{\rightarrow}
\newcommand{\lear}{\leftarrow}
\newcommand{\Riar}{\Rightarrow}
\newcommand{\Lear}{\Leftarrow}
\newcommand{\leriar}{\leftrightarrow}
\newcommand{\Leriar}{\Leftrightarrow}

\newcommand{\uC}{\underline {\bf C}}
\newcommand{\uD}{\underline {\bf D}}
\newcommand{\uE}{\underline E}
\newcommand{\ugS}{\underline\Sigma}
\newcommand{\uunion}{\underline\cup}
\newcommand{\ubigunion}{\underline\bigcup}
\newcommand{\unE}{\underline E}

\newcommand{\oE}{{\overline E}}
\newcommand{\oP}{{\overline P}}
\newcommand{\oV}{{\overline V}}
\newcommand{\oW}{{\overline W}}
\newcommand{\oU}{{\overline U}}
\newcommand{\oD}{{\overline D}}

\newcommand{\cA}{{\cal A}}
\newcommand{\cB}{{\cal B}}
\newcommand{\cC}{{\cal C}}
\newcommand{\cD}{{\cal D}}
\newcommand{\cE}{{\cal E}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cG}{{\cal G}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cJ}{{\cal J}}
\newcommand{\cL}{{\cal L}}
\newcommand{\cM}{{\cal M}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cO}{{\cal O}}
\newcommand{\cP}{{\cal P}}
\newcommand{\cR}{{\cal R}}
\newcommand{\cS}{{\cal S}}
\newcommand{\cT}{{\cal T}}
\newcommand{\cU}{{\cal U}}
\newcommand{\cV}{{\cal V}}
\newcommand{\cW}{{\cal W}}

\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}

\newcommand{\sm}{\leadsto}
\newcommand{\sopra}[2]{\stackrel{#1}{#2}}

%definitions for \bf letters
\newcommand{\bb}{{\bf b}}
\newcommand{\bA}{{\bf A}}
\newcommand{\bB}{{\bf B}}
\newcommand{\bC}{{\bf C}}
\newcommand{\bD}{{\bf D}}
\newcommand{\bE}{{\bf E}}
\newcommand{\bF}{{\bf F}}
\newcommand{\bK}{{\bf K}}
\newcommand{\bM}{{\bf M}}
\newcommand{\bN}{{\bf N}}
\newcommand{\bP}{{\bf P}}
\newcommand{\bR}{{\bf R}}
\newcommand{\bS}{{\bf S}}
\newcommand{\bT}{{\bf T}}
\newcommand{\bU}{{\bf U}}
\newcommand{\bX}{{\bf X}}
\newcommand{\bRel}{{\bf Rel}}
\newcommand{\bx}{{\bf x }}

\newcommand{\bCX}{{{\bf C}[X]}}

%definitions for lower case greek letters
\newcommand{\ga}{\alpha}
\newcommand{\gb}{\beta}
\newcommand{\gam}{\gamma}
\newcommand{\gd}{\delta}
\newcommand{\gep}{\varepsilon}
\newcommand{\gz}{\zeta}
\newcommand{\geta}{\eta}
\newcommand{\gth}{\theta}
\newcommand{\gi}{\iota}
\newcommand{\gv}{\nu}
\newcommand{\gk}{\kappa}
\newcommand{\gl}{\lambda}
\newcommand{\gm}{\mu}
\newcommand{\gn}{\nu}
\newcommand{\gx}{\xi}
\newcommand{\gp}{\pi}
\newcommand{\gr}{\rho}
\newcommand{\gs}{\sigma}
\newcommand{\gt}{\tau}
\newcommand{\gu}{\upsilon}
\newcommand{\gph}{\varphi}
\newcommand{\gch}{\chi}
\newcommand{\gps}{\psi}
\newcommand{\go}{\omega}

\newcommand{\gG}{\Gamma}
\newcommand{\gF}{\Phi}
\newcommand{\gD}{\Delta}
\newcommand{\gT}{\Theta}
\newcommand{\gP}{\Pi}
\newcommand{\gX}{\Xi}
\newcommand{\gS}{\Sigma}
\newcommand{\gO}{\Omega}
\newcommand{\gL}{\Lambda}
\newcommand\LT{\mbox{\sf LT}}
\newcommand\sfB{\mbox{\sf B}}
\newcommand\DCAI{\mbox{\sf DCA}_I}
\newcommand\RFA{\mbox{\sf RFA}}
\newcommand\RFAI{\mbox{\sf RFA}_I}
\newcommand\RFAJ{\mbox{\sf RFA}_J}
\newcommand\LAA{\mbox{\sf LAA}}
\newcommand\LAAI{\mbox{\sf LAA}_I}
\newcommand\WLAI{\mbox{\sf LAA}_I^w}
\newcommand\SWLAI{\mbox{\sf LAA}_I^{sw}}
\newcommand\LIEI{\mbox{\sf LIE}_I}
\newcommand\CLAI{\mbox{\sf LAA}_I^c}
\newcommand\CLFAI{\mbox{\sf LFA}_I^c}
\newcommand\SLAI{\mbox{\sf LAA}_I^s}
\newcommand\SSLAI{\mbox{\sf LAA}_I^{cs}}
\newcommand\OLAAI{\mbox{\sf OLAA}_I}
\newcommand\LAAIE{\mbox{\sf LAA}_I^\eta}
\newcommand\LAAJ{\mbox{\sf LAA}_J}
\newcommand\BA{\mbox{\sf BA}}
\newcommand\GSA{\mbox{\sf GSA}}
\newcommand\RGA{\mbox{\sf RGA}}
\newcommand\GA{\mbox{\sf GA}}
\newcommand\K{\mbox{\sf K}}
\newcommand\G{\mbox{\sf G}}

\newcommand\FLA{\mbox{\sf FLA}}
\newcommand\FLAI{\mbox{\sf FLA}_I}
\newcommand\FLAJ{\mbox{\sf FLA}_J}
\newcommand\LFA{\mbox{\sf LFA}}
\newcommand\LFAI{\mbox{\sf LFA}_I}
\newcommand\LFAJ{\mbox{\sf LFA}_J}
\newcommand\CA{\mbox{\sf CA}}
\newcommand\LA{\mbox{\sf LA}}
\newcommand\LM{\mbox{\sf LM}}
\newcommand{\CL}{\mbox{ \sf CL}}

\newcommand\ssk{{\bf k}}
\newcommand\sss{{\bf s}}
\newcommand\ssm{\mbox{\boldmath $m$}}
\newcommand\sse{\mbox{\boldmath $\gep$}}
\newcommand\ssi{{\bf I}}
\newcommand\ssl{\mbox{\boldmath $l$}}
\newcommand\sso{\mbox{\boldmath $1$}}
\newcommand\sst{\mbox{\boldmath $2$}}
\newcommand\ssT{{\mbox{\bf T}}}
\newcommand\ssF{{\mbox{\bf F}}}
\newcommand\ccc{\mbox{\boldmath $c$}}

\newcommand\Con{\mbox{Con}}

\newcommand\sbA{{\mbox{\bf A}}}%
\newcommand\ssbA{{\mbox{\footnotesize\bf A}}}%
\newcommand\sbB{\mbox{\boldmath $B$}}%
\newcommand\sbC{{\mathbf C}}%
\newcommand\sbD{\mbox{\boldmath $D$}}%
\newcommand\sbE{\mbox{\boldmath $E$}}%
\newcommand\sbF{{\mbox{\bf F}}}%
\newcommand\sbG{\mbox{\boldmath $G$}}%
\newcommand\sbH{\mbox{\boldmath $H$}}%
\newcommand\sbI{\mbox{\boldmath $I$}}%
\newcommand\sbJ{\mbox{\boldmath $J$}}%
\newcommand\sbK{{\bold K}}%
\newcommand\sbL{{\bold L}}%
\newcommand\sbM{\mbox{\bf M}}%
\newcommand\sbN{\mbox{\bf N}}%
\newcommand\sbO{{\bold O}}%
\newcommand\sbP{{\bold P}}%
\newcommand\sbQ{{\bold Q}}%
\newcommand\sbR{{\bold R}}%
\newcommand\sbS{{\bold S}}%
\newcommand\sbT{{\bold T}}%
\newcommand\sbU{{\bold U}}%
\newcommand\sbV{{\bold V}}%
\newcommand\sbW{{\bold W}}%
\newcommand\sbX{{\bold X}}%
\newcommand\sbY{{\bold Y}}%
\newcommand\sbZ{{\bold Z}}%


\newcommand\oa{{\overline{a}}}
\newcommand\ob{{\overline{b}}}
\newcommand\oc{{\overline{c}}}
\newcommand\od{{\overline{d}}}
\newcommand\ox{{\overline{x}}}
\newcommand\oy{{\overline{y}}}
\newcommand\ou{{\overline{u}}}
\newcommand\ov{{\overline{v}}}
\newcommand\ow{{\overline{w}}}
\newcommand\oz{{\overline{z}}}
\newcommand\oQ{{\overline{Q}}}
\newcommand\oN{{\overline{N}}}
\newcommand\oM{{\overline{M}}}
\newcommand\oR{{\overline{R}}}
\newcommand\oX{{\overline{X}}}
\newcommand\ogx{{\overline{\gx}}}
\newcommand\oempty{{\overline{\emptyset}}}

\newcommand\twohead{{\twoheadrightarrow}}

\newcommand\up{{\uparrow}}
\newcommand\down{{\downarrow}}
\newcommand\updown{{\updownarrow}}
\newcommand\si{{\leftarrow}}
\newcommand\de{{\rightarrow}}

\newcommand{\bCI}{{\bC[I]}}
\newcommand{\bDI}{{\bD[I]}}

\newcommand\sseq{{\subseteq}}
\newcommand\arrow{{\to}}

\newcommand{\A}{{\mathfrak{A}}}
\newcommand{\di}{{\diamondsuit}}

\newcommand{\Th}{{\mbox{Eq}}}
\newcommand{\Or}{{\mbox{Ord}}}

\newcommand{\sq}{{\sqsubseteq}}

\newcommand{\BS}{{\cal B}_{Sc}}
 


==> macro-duecolonne9.tex <==
% Macro di Giulio

\newcommand{\Tins}[1]{#1^{\cT-ins}}
\newcommand{\cardinality}[1]{card(#1)}% cardinality of a set 
\newcommand{\codepair}[2]{\hspace{+2pt}<\hspace{-2pt}#1,#2\hspace{-3pt}>}% code of a pair
\newcommand{\codepairmix}[2]{\hspace{+2pt}\ll\hspace{-2pt} #1,#2 \hspace{-2.5pt}\gg}% code of a pair N^* X N
\newcommand{\Visser}[1]{\mathscr{V}_{#1}}
\newcommand{\restr}{\upharpoonright}% restriction
\newcommand{\Kdn}[1]{\widehat{#1}}% restriction
\newcommand{\emptyrho}{\rho_\bot}% empty environment
\newcommand{\RE}{{\mathcal R}{\mathcal E}}% r.e. sets
\newcommand{\CORE}{{\mathcal R}{\mathcal E}^{co}}% co-r.e.
\newcommand{\Kleeneq}{\simeq}% Kleene equivalence
\newcommand{\Zero}{\textrm{Zero}}
\newcommand{\Pred}{\textrm{Pred}}
\newcommand{\Succ}{\textrm{Succ}}
\newcommand{\ecomp}{\zeta}
\newcommand{\st}{:}
\newcommand{\pow}[1]{\mathscr{P}(#1)}
\newcommand{\Intunder}[1]{\Lambda^o_{#1}}
\newcommand{\Prime}[1]{\cP(#1)}
\newcommand{\step}[2]{\varepsilon_{#1,#2}}
\newcommand{\D}{{\mathcal D}}
\newcommand{\E}{{\mathcal E}}
\newcommand{\std}[1]{\underline{#1}}
\newcommand{\cod}[1]{\ulcorner #1 \urcorner}
\newcommand{\vphi}{\varphi}
%\newcommand{\partarrow}{\rightharpoonup_p}
\newcommand{\partarrow}{\rightharpoonup}
\newcommand{\W}{{\cal W}}
\newcommand{\App}{\cF}
\newcommand{\Abs}{\lambda}
\newcommand{\compl}[1]{#1^c}
\newcommand{\domcomp}[1]{#1^{comp}}
\newcommand{\domdec}[1]{#1^{dec}}
\newcommand{\Intcomp}[1]{\left|  #1\right|^{comp}}
\newcommand{\Int}[1]{\left|  #1\right|}
\newcommand{\clup}[1]{#1\hspace{-5pt}\uparrow}
\newcommand{\cldn}[1]{#1\hspace{-5pt}\downarrow}
\newcommand{\inv}[1]{#1^{-}}
\newcommand{\partinv}[1]{#1^{-1}}
\newcommand{\img}[1]{#1^{+}}
%\renewcommand{\sup}[1]{\bigvee #1}
\renewcommand{\sup}[1]{\bigsqcup #1}
\newcommand{\Unsolvable}{\mathscr{U}}
\newcommand{\cl}[1]{\overline{#1}}
\newcommand{\seq}[1]{\overline{#1}}
\newcommand{\const}[1]{\underline{#1}}
\newcommand{\intrho}[1]{|#1|^i_\rho}
\renewcommand{\bold}[1]{{\bf #1}}
\newcommand{\compel}[1]{{\bf {\cal K}}(#1)}
\newcommand{\Appr}[1]{\c App(\textrm{$#1$})}
\newcommand{\imp}{\Rightarrow}
\newcommand{\sqle}{\sqsubseteq}
\newcommand{\BTle}{\sqsubseteq_\cB}
\newcommand{\BTeq}{=}
\newcommand{\BTsup}{\bigsqcup}
%\newcommand{\nat}{\mathbb{\omega}}
\newcommand{\nat}{\mathbb{N}}
\newcommand{\BT}{\mathcal{BT}}
\newcommand{\Base}{\mathcal{O}}

% Macro di Nino
\newtheorem{conjecture}{Conjecture}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{notation}[theorem]{Notation}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{subclaim}[theorem]{Subclaim}
\newtheorem{example}[theorem]{Example}

%
\newcommand{\ot}{\overline{t}}
\newcommand{\os}{\overline{s}}
\newcommand{\sskV}{{\bf k}\sp {\bf V}}
\newcommand{\sssV}{{\bf s}\sp{\bf V}}
\newcommand{\glV}{{\gl^{\bf V}}}
\newcommand{\cdotV}{\cdot^{\bf V}}
\newcommand{\cterm}{combinatory term}
\newcommand{\bZd}{\mbox{\bf Zd\,}}
\newcommand{\Cr}{\mbox{\rm Cr\,}}
\newcommand{\ConA}{{\bf C}{\rm on}\hspace{.01in}{\bf A}}
\newcommand{\ConB}{{\bf C}{\rm on}\hspace{.01in}{\bf B}}
\newcommand{\ConAB}{{\bf C}{\rm on}\hspace{.01in}({\bf A}$\times${\bf B})}
\newcommand{\lvar}{$\gl$-variable}
\newcommand{\bI}{{\bf I }}
%\newcommand{\qed}{$\Box$}
\newcommand{\TolA}{{\bf T}{\rm ol}\hspace{.01in}{\bf A}}
\newcommand{\FRA}{FR\hspace{.01in}{\bf A}}
\newcommand{\bnew}{\marginpar{\mbox{$\top$}}}
\newcommand{\enew}{\marginpar{\mbox{$\bot$}}}
\newcommand{\snew}{\marginpar{\mbox{$\leftarrow$}}}
\newcommand{\fnew}{\marginpar{\mbox{$\downarrow$}}}
\newcommand{\glxA}{\gl x^{\bA}}
\newcommand{\Zd}{\mbox{\rm Zd\,}}
% theorem-like commands
%

%\newtheorem{claim}{Claim}[section]
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{corollary}{Corollary}[section]
%\newtheorem{definition}{Definition}
%\newtheorem{definition}{Definition}[section]
%\newtheorem{proposition}{Proposition}[section]
%\newtheorem{lemma}{Lemma}[section]
%\newtheorem{example}{Example}[section]

\newtheorem{claimsub}{Claim}[subsection]
\newtheorem{theoremsub}{Theorem}[subsection]
\newtheorem{corollarysub}{Corollary}[subsection]
%\newtheorem{definition}{Definition}
\newtheorem{definitionsub}{Definition}[subsection]
\newtheorem{propositionsub}{Proposition}[subsection]
\newtheorem{lemmasub}{Lemma}[subsection]
\newtheorem{examplesub}{Example}[subsection]

\newtheorem{claimsubsub}{Claim}[subsubsection]
\newtheorem{theoremsubsub}{Theorem}[subsubsection]
\newtheorem{corollarysubsub}{Corollary}[subsubsection]
%\newtheorem{definition}{Definition}
\newtheorem{definitionsubsub}{Definition}[subsubsection]
\newtheorem{propositionsubsub}{Proposition}[subsubsection]
\newtheorem{lemmasubsub}{Lemma}[subsubsection]
\newtheorem{examplesubsub}{Example}[subsubsection]

\newcommand{\Over}[1]{\raisebox{-1.6mm}{{\scriptsize #1}}}
\newcommand{\SubOver}[1]{\raisebox{-0.6mm}{{\tiny #1}}}

\newcommand{\FOL}{\mbox{$L_{\omega,\omega}$}}

%\newcommand{\And}{\mbox{$\wedge$}}
%\newcommand{\Or}{\mbox{$\vee$}}
\newcommand{\Neg}{\mbox{$\neg$}}
\newcommand{\noteq}{\mbox{$\neq$}}
\newcommand{\fiproof}{\mbox{$(\Rightarrow)$}}
\newcommand{\ifproof}{\mbox{$(\Leftarrow)$}}
\newcommand{\of}{\mbox{$\in$}}
\newcommand{\notof}{\mbox{$\not\in$}}
\newcommand{\union}{\mbox{$\cup$}}
\newcommand{\intersection}{\mbox{$\cap$}}
\newcommand{\except}{\mbox{$-$}}
\newcommand{\cardof}[1]{\mbox{$|$}#1\mbox{$|$}}
\newcommand{\forevery}{\mbox{$\forall$}}
\newcommand{\therexists}{\mbox{$\exists$}}
\newcommand{\within}{\mbox{$\subseteq$}}
\newcommand{\includes}{\mbox{$\supseteq$}}
\newcommand{\product}{\mbox{$\times$}}
\newcommand{\Power}{\mbox{$\wp$}}
\newcommand{\Powernonempty}{\Power\mbox{$_{+}$}}
\newcommand{\yields}{\mbox{$\mapsto$}}
\newcommand{\comp}{\mbox{$\circ$}}
\newcommand{\emptys}{\mbox{$\emptyset$}}
\newcommand{\emptypres}{\emptys}
\newcommand{\nonabove}{\mbox{$\preceq$}}
\newcommand{\fullynonabove}{\mbox{$\sqsubseteq$}}
\newcommand{\classicallynonabove}{\mbox{$\leq$}}
\newcommand{\carrierof}[1]{\mbox{$|$}#1\mbox{$|$}}
\newcommand{\setof}[1]{\mbox{$\{$}#1\mbox{$\}$}}
\newcommand{\suchthat}{\mbox{$|$}}
\newcommand{\unionall}[3]{\mbox{$\bigcup_{#1\in#2}$}#3}
\newcommand{\widunionall}[3]{\parbox[t]{#3}
                         {\centering\mbox{$\bigcup$}
                          \\ \protect\vspace*{-1.5mm}
                          {\scriptsize #1\of#2}}}
\newcommand{\intsnall}[3]{\mbox{$\bigcap_{#1\in#2}$}#3}
\newcommand{\widintsnall}[3]{\parbox[t]{#3}
                         {\centering\mbox{$\bigcap$}
                          \\ \protect\vspace*{-1.5mm}
                          {\scriptsize #1\of#2}}}
\newcommand{\ifamily}[3]{\setof{#1\mbox{$_{#2}$}}\mbox{$_{#2\in#3}$}}
\newcommand{\indx}{{\it j}}
\newcommand{\anindx}{{\it k}}
\newcommand{\indxset}{{\it J}}
\newcommand{\iso}{\mbox{$\simeq$}}
\newcommand{\lweq}{\mbox{$\leq$}}
\newcommand{\greq}{\mbox{$\geq$}}
\newcommand{\grth}{\mbox{$>$}}
\newcommand{\eqdef}{\mbox{$\stackrel{\it def}{=}$}}
\newcommand{\inverseof}[1]{#1\mbox{$^{-1}$}}
\newcommand{\minverseof}[1]{#1^{-1}}

\newcommand{\seqof}[3]{#1\mbox{$_{1}$}#2\ldots#2#1\mbox{$_{#3}$}}

\newcommand{\seqSubOverof}[3]{#1\raisebox{-2.2mm}
                                     {{\tiny 1}}#2\ldots#2#1\raisebox{-2.2mm}
                                                                 {{\tiny #3}}}

\newcommand{\rpsreq}{(\dag)}
\newcommand{\epsreq}{(\ddag)}
\newcommand{\satinv}{(\S)}
\newcommand{\adequacy}{(\S\S)}
\newcommand{\fulladequacy}{(\S\S\S)}
\newcommand{\finitarity}{(\pounds)}

\newcommand{\upar}{\uparrow}
\newcommand{\Upar}{\Uparrow}
\newcommand{\doar}{\downarrow}
\newcommand{\Doar}{\Downarrow}

\newcommand{\riar}{\rightarrow}
\newcommand{\lear}{\leftarrow}
\newcommand{\Riar}{\Rightarrow}
\newcommand{\Lear}{\Leftarrow}
\newcommand{\leriar}{\leftrightarrow}
\newcommand{\Leriar}{\Leftrightarrow}

\newcommand{\uC}{\underline {\bf C}}
\newcommand{\uD}{\underline {\bf D}}
\newcommand{\uE}{\underline E}
\newcommand{\ugS}{\underline\Sigma}
\newcommand{\uunion}{\underline\cup}
\newcommand{\ubigunion}{\underline\bigcup}
\newcommand{\unE}{\underline E}

\newcommand{\oE}{{\overline E}}
\newcommand{\oP}{{\overline P}}
\newcommand{\oV}{{\overline V}}
\newcommand{\oW}{{\overline W}}
\newcommand{\oU}{{\overline U}}
\newcommand{\oD}{{\overline D}}

\newcommand{\cA}{{\cal A}}
\newcommand{\cB}{{\cal B}}
\newcommand{\cC}{{\cal C}}
\newcommand{\cD}{{\cal D}}
\newcommand{\cE}{{\cal E}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cG}{{\cal G}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cJ}{{\cal J}}
\newcommand{\cL}{{\cal L}}
\newcommand{\cM}{{\cal M}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cO}{{\cal O}}
\newcommand{\cP}{{\cal P}}
\newcommand{\cR}{{\cal R}}
\newcommand{\cS}{{\cal S}}
\newcommand{\cT}{{\cal T}}
\newcommand{\cU}{{\cal U}}
\newcommand{\cV}{{\cal V}}
\newcommand{\cW}{{\cal W}}

\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}

\newcommand{\sm}{\leadsto}
\newcommand{\sopra}[2]{\stackrel{#1}{#2}}

%definitions for \bf letters
\newcommand{\bb}{{\bf b}}
\newcommand{\bA}{{\bf A}}
\newcommand{\bB}{{\bf B}}
\newcommand{\bC}{{\bf C}}
\newcommand{\bD}{{\bf D}}
\newcommand{\bE}{{\bf E}}
\newcommand{\bF}{{\bf F}}
\newcommand{\bK}{{\bf K}}
\newcommand{\bM}{{\bf M}}
\newcommand{\bN}{{\bf N}}
\newcommand{\bP}{{\bf P}}
\newcommand{\bR}{{\bf R}}
\newcommand{\bS}{{\bf S}}
\newcommand{\bT}{{\bf T}}
\newcommand{\bU}{{\bf U}}
\newcommand{\bX}{{\bf X}}
\newcommand{\bRel}{{\bf Rel}}
\newcommand{\bx}{{\bf x }}

\newcommand{\bCX}{{{\bf C}[X]}}

%definitions for lower case greek letters
\newcommand{\ga}{\alpha}
\newcommand{\gb}{\beta}
\newcommand{\gam}{\gamma}
\newcommand{\gd}{\delta}
\newcommand{\gep}{\varepsilon}
\newcommand{\gz}{\zeta}
\newcommand{\geta}{\eta}
\newcommand{\gth}{\theta}
\newcommand{\gi}{\iota}
\newcommand{\gv}{\nu}
\newcommand{\gk}{\kappa}
\newcommand{\gl}{\lambda}
\newcommand{\gm}{\mu}
\newcommand{\gn}{\nu}
\newcommand{\gx}{\xi}
\newcommand{\gp}{\pi}
\newcommand{\gr}{\rho}
\newcommand{\gs}{\sigma}
\newcommand{\gt}{\tau}
\newcommand{\gu}{\upsilon}
\newcommand{\gph}{\varphi}
\newcommand{\gch}{\chi}
\newcommand{\gps}{\psi}
\newcommand{\go}{\omega}

\newcommand{\gG}{\Gamma}
\newcommand{\gF}{\Phi}
\newcommand{\gD}{\Delta}
\newcommand{\gT}{\Theta}
\newcommand{\gP}{\Pi}
\newcommand{\gX}{\Xi}
\newcommand{\gS}{\Sigma}
\newcommand{\gO}{\Omega}
\newcommand{\gL}{\Lambda}
\newcommand\LT{\mbox{\sf LT}}
\newcommand\sfB{\mbox{\sf B}}
\newcommand\DCAI{\mbox{\sf DCA}_I}
\newcommand\RFA{\mbox{\sf RFA}}
\newcommand\RFAI{\mbox{\sf RFA}_I}
\newcommand\RFAJ{\mbox{\sf RFA}_J}
\newcommand\LAA{\mbox{\sf LAA}}
\newcommand\LAAI{\mbox{\sf LAA}_I}
\newcommand\WLAI{\mbox{\sf LAA}_I^w}
\newcommand\SWLAI{\mbox{\sf LAA}_I^{sw}}
\newcommand\LIEI{\mbox{\sf LIE}_I}
\newcommand\CLAI{\mbox{\sf LAA}_I^c}
\newcommand\CLFAI{\mbox{\sf LFA}_I^c}
\newcommand\SLAI{\mbox{\sf LAA}_I^s}
\newcommand\SSLAI{\mbox{\sf LAA}_I^{cs}}
\newcommand\OLAAI{\mbox{\sf OLAA}_I}
\newcommand\LAAIE{\mbox{\sf LAA}_I^\eta}
\newcommand\LAAJ{\mbox{\sf LAA}_J}
\newcommand\BA{\mbox{\sf BA}}
\newcommand\GSA{\mbox{\sf GSA}}
\newcommand\RGA{\mbox{\sf RGA}}
\newcommand\GA{\mbox{\sf GA}}
\newcommand\K{\mbox{\sf K}}
\newcommand\G{\mbox{\sf G}}

\newcommand\FLA{\mbox{\sf FLA}}
\newcommand\FLAI{\mbox{\sf FLA}_I}
\newcommand\FLAJ{\mbox{\sf FLA}_J}
\newcommand\LFA{\mbox{\sf LFA}}
\newcommand\LFAI{\mbox{\sf LFA}_I}
\newcommand\LFAJ{\mbox{\sf LFA}_J}
\newcommand\CA{\mbox{\sf CA}}
\newcommand\LA{\mbox{\sf LA}}
\newcommand\LM{\mbox{\sf LM}}
\newcommand{\CL}{\mbox{ \sf CL}}

\newcommand\ssk{{\bf k}}
\newcommand\sss{{\bf s}}
\newcommand\ssm{\mbox{\boldmath $m$}}
\newcommand\sse{\mbox{\boldmath $\gep$}}
\newcommand\ssi{{\bf i}}
\newcommand\ssl{\mbox{\boldmath $l$}}
\newcommand\sso{\mbox{\boldmath $1$}}
\newcommand\sst{\mbox{\boldmath $2$}}
\newcommand\ssT{{\mbox{\boldmath T}}}
\newcommand\ssF{{\mbox{\boldmath F}}}
\newcommand\ccc{\mbox{\boldmath $c$}}

\newcommand\Con{\mbox{Con}}

\newcommand\sbA{{\mbox{\bf A}}}%
\newcommand\ssbA{{\mbox{\footnotesize\bf A}}}%
\newcommand\sbB{\mbox{\boldmath $B$}}%
\newcommand\sbC{{\mathbf C}}%
\newcommand\sbD{\mbox{\boldmath $D$}}%
\newcommand\sbE{\mbox{\boldmath $E$}}%
\newcommand\sbF{{\mbox{\bf F}}}%
\newcommand\sbG{\mbox{\boldmath $G$}}%
\newcommand\sbH{\mbox{\boldmath $H$}}%
\newcommand\sbI{\mbox{\boldmath $I$}}%
\newcommand\sbJ{\mbox{\boldmath $J$}}%
\newcommand\sbK{{\bold K}}%
\newcommand\sbL{{\bold L}}%
\newcommand\sbM{\mbox{\bf M}}%
\newcommand\sbN{\mbox{\bf N}}%
\newcommand\sbO{{\bold O}}%
\newcommand\sbP{{\bold P}}%
\newcommand\sbQ{{\bold Q}}%
\newcommand\sbR{{\bold R}}%
\newcommand\sbS{{\bold S}}%
\newcommand\sbT{{\bold T}}%
\newcommand\sbU{{\bold U}}%
\newcommand\sbV{{\bold V}}%
\newcommand\sbW{{\bold W}}%
\newcommand\sbX{{\bold X}}%
\newcommand\sbY{{\bold Y}}%
\newcommand\sbZ{{\bold Z}}%


\newcommand\oa{{\overline{a}}}
\newcommand\ob{{\overline{b}}}
\newcommand\oc{{\overline{c}}}
\newcommand\od{{\overline{d}}}
\newcommand\ox{{\overline{x}}}
\newcommand\oy{{\overline{y}}}
\newcommand\ou{{\overline{u}}}
\newcommand\ov{{\overline{v}}}
\newcommand\ow{{\overline{w}}}
\newcommand\oz{{\overline{z}}}
\newcommand\oQ{{\overline{Q}}}
\newcommand\oN{{\overline{N}}}
\newcommand\oM{{\overline{M}}}
\newcommand\oR{{\overline{R}}}
\newcommand\oX{{\overline{X}}}
\newcommand\ogx{{\overline{\gx}}}
\newcommand\oempty{{\overline{\emptyset}}}

\newcommand\twohead{{\twoheadrightarrow}}

\newcommand\up{{\uparrow}}
\newcommand\down{{\downarrow}}
\newcommand\updown{{\updownarrow}}
\newcommand\si{{\leftarrow}}
\newcommand\de{{\rightarrow}}

\newcommand{\bCI}{{\bC[I]}}
\newcommand{\bDI}{{\bD[I]}}

\newcommand\sseq{{\subseteq}}
\newcommand\arrow{{\to}}

\newcommand{\A}{{\mathfrak{A}}}
\newcommand{\di}{{\diamondsuit}}

\newcommand{\Th}{{\mbox{Eq}}}
\newcommand{\Or}{{\mbox{Ord}}}

\newcommand{\sq}{{\sqsubseteq}}

\newcommand{\BS}{{\cal B}_{Sc}}
 

